PolyFormer: Referring Image Segmentation as Sequential Polygon Generation

In this work, instead of directly predicting the pixel-level segmentation masks, the problem of referring image segmentation is formulated as sequential polygon generation, and the predicted polygons can be later converted into segmentation masks. This is enabled by a new sequence-to-sequence framework, Polygon Transformer (PolyFormer), which takes a sequence of image patches and text query tokens as input, and outputs a sequence of polygon vertices autoregressively. For more accurate geometric localization, we propose a regression-based decoder, which predicts the precise floating-point coordinates directly, without any coordinate quantization error. In the experiments, PolyFormer outperforms the prior art by a clear margin, e.g., 5.40% and 4.52% absolute improvements on the challenging RefCOCO+ and RefCOCOg datasets. It also shows strong generalization ability when evaluated on the referring video segmentation task without fine-tuning, e.g., achieving competitive 61.5% J&F on the Ref-DAVIS17 dataset.

==> figs/attn.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \begin{tabular}[b]{cccccc}
        % \hline
         
        \multicolumn{6}{l}{Expression: ``an Asian girl with a pink shirt eating at the table"} \\
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/3_1_step_0_37.75390625.png}
        \caption{$t=0, \ \hat{x}_{min}=37.75$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
            \includegraphics[width=\textwidth]{figs/attn/3_1_step_1_169.921875.png}
        \caption{$t=1, \ \hat{y}_{min}=169.92$}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/3_1_step_2_192.8125.png}
        \caption{$t=2,\ \hat{x}_{max}=192.81$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/3_1_step_3_351.5625.png}
        \caption{$t=3,\ \hat{y}_{max}=351.56$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/3_1_step_54_104.296875.png}
        \caption{$t=54,\ \hat{x}_1^{26}=104.30$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/3_1_step_55_195.703125.png}
        \caption{$t=55,\ \hat{y}_1^{26}=195.70$}
        \end{subfigure} \\ 
        
        \multicolumn{6}{l}{Expression: ``a sandwich which is roughly triangular in shape"} \\
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/82_0_step_0_0.07375860214233398.png}
        \caption{$t=0, \ \hat{x}_b^1=0.07$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
            \includegraphics[width=\textwidth]{figs/attn/82_0_step_1_185.1240234375.png}
        \caption{$t=1, \ \hat{y}_b^1=185.12$}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/82_0_step_2_371.443359375.png}
        \caption{$t=2,\ \hat{x}_b^2=371.44$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/82_0_step_3_484.1015625.png}
        \caption{$t=3,\ \hat{y}_b^2=484.10$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/82_0_step_58_24.989501953125.png}
        \caption{$t=58,\ \hat{x}_1^{28}=25.00$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn/82_0_step_59_478.72265625.png}
        \caption{$t=59,\ \hat{y}_1^{28}=478.72$}
        \end{subfigure} \\ 
        %_pred_overlayed.png
        

        % \hline
    \end{tabular}
    \caption{Visualization of averaged cross-attention map in PolyFormer decoder at inference step $t$. }
    \label{fig:attn}
\end{figure*}

==> figs/attn_v2.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \begin{tabular}[b]{cccccc}
        % \hline
         
        \multicolumn{6}{l}{Expression: ``an Asian girl with a pink shirt eating at the table"} \\
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/3_1_step_4_118.75.png}
        \caption{$t_{poly}=0$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
            \includegraphics[width=\textwidth]{figs/attn_v2/3_1_step_17_260.15625.png}
        \caption{$t_{poly}=13$}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/3_1_step_27_345.703125.png}
        \caption{$t_{poly}=23$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/3_1_step_37_332.109375.png}
        \caption{$t_{poly}=33$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/3_1_step_47_263.4375.png}
        \caption{$t_{poly}=43$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/3_1_step_55_195.703125.png}
        \caption{$t_{poly}=51$}
        \end{subfigure} \\ 
        
        \multicolumn{6}{l}{Expression: ``a chili dog with slices of cheese visible under the chili"} \\
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/15_0_step_4_164.21875.png}
        \caption{$t_{poly}=0$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
            \includegraphics[width=\textwidth]{figs/attn_v2/15_0_step_14_265.625.png}
        \caption{$t_{poly}=10$}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/15_0_step_21_265.3125.png}
        \caption{$t_{poly}=17$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/15_0_step_31_405.9375.png}
        \caption{$t_{poly}=27$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/15_0_step_49_451.875.png}
        \caption{$t_{poly}=45$}
        \end{subfigure} &
        \begin{subfigure}[b]{0.165\linewidth}
        \includegraphics[width=\textwidth]{figs/attn_v2/15_0_step_69_186.9140625.png}
        \caption{$t_{poly}=65$}
        \end{subfigure} \\ 
        

        % \hline
    \end{tabular}
    % \caption{Visualization of averaged cross-attention map in PolyFormer decoder at inference step $t_{poly}$ for polygon prediction. The last column corresponds to the last inference step.}
    \caption{Decoder's cross-attention map when predicting the polygons. The first and last columns visualize the first and last predicted vertex coordinate tokens, respectively.}
    \label{fig:attn}
\end{figure*}

==> figs/failure.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \setlength{\tabcolsep}{0.8mm}{\begin{tabular}[b]{lcccccc}
    
        \rotatebox{90}{\hskip 2em Prediction}&
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/failure/75_0_poly_2d_large.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/failure/3392_0_one half of a sandwich leaning against a whole sandwich_pred_overlayed.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/failure/1061_0_white and black suitcase chained to 2 other suitcases_pred_overlayed.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/failure/100_1_a zebra standing between two fighting zebras_pred_overlayed.png}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/failure/4835_1_giraffe laying to west_pred_overlayed.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/failure/482_0_a minivan that serves as a taxi cab_pred_overlayed.png}
        \end{subfigure} \\ 
        
        \rotatebox{90}{\hskip 2em Ground-truth}&
        \begin{subfigure}[t]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/failure/75_0_gt.png}
        \caption{(a) ``the midsized vase"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/failure/3392_0_one half of a sandwich leaning against a whole sandwich_gt_overlayed.png}
            \caption{(b) ``one half of a sandwich leaning against a whole sandwich"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/failure/1061_0_white and black suitcase chained to 2 other suitcases_gt_overlayed.png}
        \caption{(d) ``white and black suitcase chained to 2 other suitcases"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/failure/100_1_a zebra standing between two fighting zebras_gt_overlayed.png}
            \caption{(e) ``a zebra standing between two fighting zebras"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/failure/4835_1_giraffe laying to west_gt_overlayed.png}
            \caption{(c) ``giraffe laying to west"}
        \end{subfigure} &  
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/failure/482_0_a minivan that serves as a taxi cab_gt_overlayed.png}
            \caption{(f) ``a minivan that serves as a taxi cab"}
        \end{subfigure}\\ 
        
        
        %Input Image & LAVT~\cite{yang2022lavt} & SeqTR~\cite{zhu2022seqtr} & PolyFormer (ours)  &  Ground-truth \\

        % \hline
    \end{tabular}}
    \caption{Failure case visualization.}
    % \caption{Visualization results on RefCOCOg. Our unified framework is able to detect and segment the referred object simultaneously. }
    \label{fig:failure}
    %\vspace{-1.5em}
\end{figure*}


% \begin{tblr}{
%   colspec = {Q[b,4em]|Q[c,m]}
% }
%   LAVT~\cite{yang2022lavt} & \includegraphics[width=0.18\textwidth]{figs/visualization_2/449_1_lavt.png}\\
% \end{tblr}

==> figs/visualization.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \begin{tabular}[b]{ccccc}
        % \hline
         
        \multicolumn{5}{l}{Expression: ``a cow that is \textit{\textbf{being fed}} by a bottle"} \\
        \begin{subfigure}[b]{0.2\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization/2001_1_a cow that is being fed by a bottle.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/2001_1_lavt.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/2001_1_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/2001_1_poly_1d_base.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/2001_1_gt.png}
        \end{subfigure}\\ 
        
        % \multicolumn{5}{l}{Expression: ``a \textit{\textbf{red and black}} motorcycle with a \textit{\textbf{Santa}} riding it"} \\
        % \begin{subfigure}[b]{0.2\linewidth}
        % \includegraphics[width=\textwidth]{figs/visualization/1993_1_a red and black motorcycle with a santa riding it.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/1993_1_lavt.png}
        % \end{subfigure} &  
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/1993_1_seqtr.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/1993_1_poly_1d_base.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/1993_1_gt.png}
        % \end{subfigure}\\ 
        
        % \multicolumn{5}{l}{Expression: ``a \textit{\textbf{without hairy brown}} color teddy bear"} \\
        % \begin{subfigure}[b]{0.2\linewidth}
        % \includegraphics[width=\textwidth]{figs/visualization/10_1_a without hairy brown color teddy bear.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/10_1_lavt.png}
        % \end{subfigure} &  
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/10_1_seqtr.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/10_1_poly_1d_base.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/10_1_gt.png}
        %\end{subfigure}\\ 
        % \multicolumn{5}{l}{Expression: ``boy with blue plaid shirt and glasses"} \\
        % \begin{subfigure}[b]{0.2\linewidth}
        % \includegraphics[width=\textwidth]{figs/visualization/822_0_boy with blue plaid shirt and glasses.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/822_0_lavt.png}
        % \end{subfigure} &  
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/822_0_seqtr.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/822_0_poly_1d_base.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.2\linewidth}
        %     \includegraphics[width=\textwidth]{figs/visualization/822_0_gt.png}
        % \end{subfigure}\\ 
        
        \multicolumn{5}{l}{Expression: ``a \textit{\textbf{dark grey}} dog \textit{\textbf{on}} a light grey round bed \textit{\textbf{wearing}} a red collar"} \\
        \begin{subfigure}[b]{0.2\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization/1987_0_a dark grey dog on a light grey round bed wearing a red collar.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/1987_0_lavt.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/1987_0_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/1987_0_poly_1d_base.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/1987_0_gt.png}
        \end{subfigure}\\ 
        
        \multicolumn{5}{l}{Expression: ``a woman \textit{\textbf{standing next}} to the drum set"} \\
        \begin{subfigure}[b]{0.2\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization/775_0_a woman standing next to the drum set.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/775_0_lavt.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/775_0_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/775_0_poly_1d_base.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.2\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization/775_0_gt.png}
        \end{subfigure}\\ 
        
        
        Input Image & LAVT~\cite{yang2022lavt} & SeqTR~\cite{zhu2022seqtr} & PolyFormer (ours)  &  Ground-truth \\

        % \hline
    \end{tabular}
    \caption{Visual comparisons between LAVT~
    \cite{yang2022lavt}, SeqTR~\cite{zhu2022seqtr} and PolyFormer on RefCOCOg test set. PolyFormer simultaneously predicts the bounding box and polygon vertices that forms the segmentation mask. 
    % Blue point indicates the starting point of the vertex sequence. 
    LAVT is for referring image segmentation only. For SeqTR, we generate the bounding boxes and segmentation masks from the task-specific models as they perform better than the multi-task model.}
    % \caption{Visualization results on RefCOCOg. Our unified framework is able to detect and segment the referred object simultaneously. }
    \label{fig:visualization}
    %\vspace{-1.5em}
\end{figure*}

==> figs/visualization_2.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \setlength{\tabcolsep}{0.8mm}{\begin{tabular}[b]{lccccc}
        % \hline
         
        %\multicolumn{5}{l}{Expression: ``a cow that is \textit{\textbf{being fed}} by a bottle"} \\
        \rotatebox{90}{\hskip 3em LAVT~\cite{yang2022lavt}} &
        \begin{subfigure}[b]{0.1239\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_2/449_1_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1073_1_lavt.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1246_1_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1365_0_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1407_0_lavt.png}
        \end{subfigure}\\ 
        
        \rotatebox{90}{\hskip 3em SeqTR~\cite{zhu2022seqtr}}&
        \begin{subfigure}[b]{0.1239\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_2/449_1_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1073_1_seqtr.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1246_1_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1365_0_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1407_0_seqtr.png}
        \end{subfigure}\\ 
        
        \rotatebox{90}{\hskip 1.5em  \textbf{PolyFormer}}&
        \begin{subfigure}[t]{0.1239\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_2/449_1_poly_2d_large.png}
        \caption{``horse on the left of the group of horses"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1073_1_poly_2d_large.png}
            \caption{``the elephant with the baby elephant"}
        \end{subfigure} &  
        \begin{subfigure}[t]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1246_1_poly_2d_large.png}
            \caption{``a woman wearing jeans holding a laptop sitting in between two other women"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1365_0_poly_2d_large.png}
            \caption{``a black car parked at a transportation terminal"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.1239\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1407_0_poly_2d_large.png}
            \caption{``girl in purple"}
        \end{subfigure}\\ 
        
        
        
        %Input Image & LAVT~\cite{yang2022lavt} & SeqTR~\cite{zhu2022seqtr} & PolyFormer (ours)  &  Ground-truth \\

        % \hline
    \end{tabular}}
    \caption{Visual comparisons between LAVT~
    \cite{yang2022lavt}, SeqTR~\cite{zhu2022seqtr} and PolyFormer on RefCOCOg test set. PolyFormer simultaneously predicts the bounding box and polygon vertices that forms the segmentation mask. 
    % Blue point indicates the starting point of the vertex sequence. 
    LAVT is for referring image segmentation only. For SeqTR, we generate the bounding boxes and segmentation masks from the task-specific models as they perform better than the multi-task model.}
    % \caption{Visualization results on RefCOCOg. Our unified framework is able to detect and segment the referred object simultaneously. }
    \label{fig:visualization}
    %\vspace{-1.5em}
\end{figure*}


% \begin{tblr}{
%   colspec = {Q[b,4em]|Q[c,m]}
% }
%   LAVT~\cite{yang2022lavt} & \includegraphics[width=0.18\textwidth]{figs/visualization_2/449_1_lavt.png}\\
% \end{tblr}

==> figs/visualization_supp_2.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \setlength{\tabcolsep}{0.8mm}{\begin{tabular}[b]{lcccccc}
        % \hline
         
        %\multicolumn{5}{l}{Expression: ``a cow that is \textit{\textbf{being fed}} by a bottle"} \\
        
        
        \rotatebox{90}{\hskip 3em LAVT~\cite{yang2022lavt}} &
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_supp_2/136_0_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/822_0_lavt.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/1572_0_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/1987_0_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/5019_1_lavt.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1407_0_lavt.png}
        \end{subfigure} \\ 
        
        \rotatebox{90}{\hskip 3em SeqTR~\cite{zhu2022seqtr}}&
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_supp_2/136_0_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_supp_2/822_0_seqtr.png}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/1572_0_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/1987_0_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/5019_1_seqtr.png}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1407_0_seqtr.png}
        \end{subfigure}\\ 
        
        \rotatebox{90}{\hskip 1.5em  \textbf{PolyFormer}}&
        \begin{subfigure}[t]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/visualization_supp_2/136_0_poly_2d_large.png}
        \caption{``old yellow and white truck parked behind other truck"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/822_0_poly_2d_large.png}
            \caption{``boy with blue plaid shirt and glasses"}
        \end{subfigure} &  
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/1572_0_poly_2d_large.png}
            \caption{``the surfboard the woman in a white shirt and blue capris is holding"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/1987_0_poly_2d_large.png}
            \caption{``a dark grey dog on a light grey round bed wearing a red collar"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_supp_2/5019_1_poly_2d_large.png}
            \caption{``a girl was cooking the food and serving"}
        \end{subfigure} & 
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/visualization_2/1407_0_poly_2d_large.png}
            \caption{``girl in purple"}
        \end{subfigure}\\ 
        
        
        %Input Image & LAVT~\cite{yang2022lavt} & SeqTR~\cite{zhu2022seqtr} & PolyFormer (ours)  &  Ground-truth \\

        % \hline
    \end{tabular}}
    \caption{Visual comparisons between LAVT~
    \cite{yang2022lavt}, SeqTR~\cite{zhu2022seqtr} and PolyFormer on RefCOCOg test set. PolyFormer simultaneously predicts the bounding box and polygon vertices that forms the segmentation mask. 
    % Blue point indicates the starting point of the vertex sequence. 
    LAVT is for referring image segmentation only. For SeqTR, we generate the bounding boxes and segmentation masks from the task-specific models as they perform better than the multi-task model.}
    % \caption{Visualization results on RefCOCOg. Our unified framework is able to detect and segment the referred object simultaneously. }
    \label{fig:visualization_supp_2}
    %\vspace{-1.5em}
\end{figure*}


% \begin{tblr}{
%   colspec = {Q[b,4em]|Q[c,m]}
% }
%   LAVT~\cite{yang2022lavt} & \includegraphics[width=0.18\textwidth]{figs/visualization_2/449_1_lavt.png}\\
% \end{tblr}

==> figs/zeroshot.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \setlength{\tabcolsep}{0.8mm}{\begin{tabular}[b]{lccccc}
        % \hline
         
        %\multicolumn{5}{l}{Expression: ``a cow that is \textit{\textbf{being fed}} by a bottle"} \\
        
        % \rotatebox{90}{\hskip 3em Input}&
        % \begin{subfigure}[b]{0.15\linewidth}
        % \includegraphics[width=\textwidth]{figs/zero_shot/a gentleman otter in a 19th century portrait.png}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.15\linewidth}
        %     \includegraphics[width=\textwidth]{figs/zero_shot/A pikachu fine dining with a view to the Eiffel Tower.jpeg}
        % \end{subfigure} &  
        % \begin{subfigure}[b]{0.15\linewidth}
        %     \includegraphics[width=\textwidth]{figs/zero_shot/A small cabin on top of a snowy mountain in the style of Disney artstation.jpeg}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.15\linewidth}
        %     \includegraphics[width=\textwidth]{figs/zero_shot/A shiba inu puppy painted by monet.jpeg}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.15\linewidth}
        %     \includegraphics[width=\textwidth]{figs/zero_shot/pig.jpeg}
        % \end{subfigure}\\ 
        
        \rotatebox{90}{\hskip 3em LAVT~\cite{yang2022lavt}} &
        \begin{subfigure}[b]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/zero_shot/otta_lavt.jpeg}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/pikachu_lavt.jpeg}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/cabin_lavt.jpeg}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/shiba_lavt.jpeg}
        \end{subfigure} &
        \begin{subfigure}[b]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/pig_lavt.jpeg}
        \end{subfigure}\\ 
        
        
        \rotatebox{90}{\hskip 1.5em  \textbf{PolyFormer}}&
        \begin{subfigure}[t]{0.15\linewidth}
        \includegraphics[width=\textwidth]{figs/zero_shot/otta_poly_2d_large.png}
        \caption{``A gentleman otter in a 19th century portrait"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/pikachu_poly_2d_large.png}
            \caption{``A pikachu fine dining with a view to the Eiffel Tower"}
        \end{subfigure} &  
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/cabin_poly_2d_large.png}
            \caption{``A small cabin on top of a snowy mountain in the style of Disney artstation"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/shiba_poly_2d_large.png}
            \caption{``A shiba inu puppy painted by Monet"}
        \end{subfigure} &
        \begin{subfigure}[t]{0.15\linewidth}
            \includegraphics[width=\textwidth]{figs/zero_shot/pig_poly_2d_large .png}
            \caption{``A pig robot preparing a delicious meal"}
        \end{subfigure}\\ 
        
        
        
        %Input Image & LAVT~\cite{yang2022lavt} & SeqTR~\cite{zhu2022seqtr} & PolyFormer (ours)  &  Ground-truth \\

        % \hline
    \end{tabular}}
    \caption{Visual comparisons between LAVT~
    \cite{yang2022lavt} and PolyFormer on synthetic images generated by stable diffusion~\cite{rombach2021highresolution}.}
    \label{fig:zero-shot}
    %\vspace{-1.5em}
\end{figure*}


% \begin{tblr}{
%   colspec = {Q[b,4em]|Q[c,m]}
% }
%   LAVT~\cite{yang2022lavt} & \includegraphics[width=0.18\textwidth]{figs/visualization_2/449_1_lavt.png}\\
% \end{tblr}

==> tables/davis_2.tex <==
\begin{table}[htbp]
\centering
\scalebox{0.9}{\setlength{\tabcolsep}{0.8mm}{\begin{tabular}{l|c|c|c}
\toprule
Decoder            &RefCOCO & RefCOCO+   & RefCOCOg    \\
\midrule
% \hline
\multicolumn{4}{l}{Referring Image Segmentation} \\
\midrule
% CMSA~\cite{ye2019cross} & 34.7 & 32.2 & 37.2  \\
% CMSA+RNN ~\cite{ye2019cross} & 40.2 & 36.9 & 43.5 \\
% URVOS~\cite{seo2020urvos}              & 51.5  & 47.3  & 56.0     \\
% CMPC-V~\cite{liu2021cross} & - & - & -  \\
% ClawCraneNet~\cite{liang2021clawcranenet} & - & - & -   \\
% MTTR ~\cite{botach2022mttr} & - & - & -  \\
Classification       & 74.11  & 68.79  & 67.69   \\
\midrule
% PolyFormer$^*$ (Ours) & 60.8 & 56.3 & 65.3 &  69.9 \\
% PolyFormer-B-2D$^*$ (Ours)  & 58.8 & 54.6 & 63.0  \\
\textbf{Regression} & \textbf{75.96}\small{ (+1.85)} & \textbf{70.65}\small{ (+1.86)}& \textbf{69.36}\small{ (+1.67)} \\
% PolyFormer-L-2D$^*$ (Ours)  & 61.3  & 57.1 & 65.5 \\
\midrule
% \hline
\multicolumn{4}{l}{Referring Expression Comprehension} \\
\midrule
Classification       & 87.03 & 81.35  & 82.21   \\
\midrule
% PolyFormer$^*$ (Ours) & 60.8 & 56.3 & 65.3 &  69.9 \\
% PolyFormer-B-2D$^*$ (Ours)  & 58.8 & 54.6 & 63.0  \\
\textbf{Regression} & \textbf{89.73}\small{ (+2.70)} & \textbf{83.73}\small{ (+2.38)}& \textbf{84.46}\small{ (+2.25)} \\
% PolyFormer-L-2D$^*$ (Ours)  & 61.3  & 57.1 & 65.5 \\
\bottomrule
\end{tabular}}}
\caption{Ablation study on classification \textit{v.s.} regression-based decoder. 
% \zc{I would say classification v.s. regression. Using PolyFormer, the readers don't see what you ablate here.}\hd{fixed}
} 
\label{tab:decoder}
\end{table}

==> tables/rec.tex <==
\begin{table*}[t]
   \centering
    %   \caption{Comparison with state-of-the-art methods in terms of Acc@0.5 on three benchmark datasets for the REC task. Following~\cite{yang2022lavt}, we refer to the language model of each reference method as the main learnable function that transforms word embeddings before multi-modal feature fusion. RN101 and RN152 denotes ResNet-101 and ResNet-152~\cite{he2016deep}, WRN101 refers to Wide ResNet-101~\cite{zagoruyko2016wide}, ENB3 denotes EfficientNetB3~\cite{enb3} and DN53 refers to Darknet-53~\cite{redmon2018yolov3}.}
   \scalebox{0.95}{\setlength{\tabcolsep}{2.0mm}{\begin{tabular}{l|l|l|c|c|c|c|c|c|c|c}
      \toprule[1pt]
      \multirow{2}{*}{Method} & Visual &
      Text & 
      \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
      \cline{4-11}
                                    & Backbone & Encoder & val   & test A & test B & val & test A & test B & val & test  \\
      \hline
    %   MAttNet~\cite{yu2018mattnet} & RN101 & Bi-LSTM & 76.65 & 81.14 & 69.99 & 65.33 & 71.62 & 56.02 & 66.58 & 67.27 \\ 
      UNTIER-L~\cite{chen2020uniter} & RN101 & BERT & 81.41 & 87.04 & 74.17 & 75.90 & 81.45 & 66.70 & 74.86 & 75.77 \\
      VILLA-L~\cite{gan2020large} & RN101 & BERT & 82.39 & 87.48 & 74.84 & 76.17 & 81.54 & 66.84 & 76.18 & 76.71 \\
      RefTr~\cite{li2021referring} & RN101 & BERT-base & 85.65 & 88.73 & 81.16 & 77.55 & 82.26 & 68.99 & 79.25 & 80.01 \\ 
    SeqTR~\cite{zhu2022seqtr} & DN53 & Bi-GRU & 87.00 & 90.15 & 83.59 & 78.69 & 84.51 & 71.87 & 82.69 & 83.37 \\
      MDETR~\cite{kamath2021mdetr} & ENB3 & RoBERTa-base & 87.51 & 90.40 & 82.67 & 81.13 & 85.52 & 72.96 & 83.35 & 83.31\\
      OFA-B~\cite{wang2022unifying} & RN101 & 
      Embedding layer &  88.48 & 90.67 & 83.30 & 81.39 & 87.15 & 74.29 & 82.29 & 82.31 \\
    UniTAB~\cite{yang2022unitab} & RN101 & RoBERT-base & 88.59 & 91.06 & 83.75 & 80.97 & 85.36 & 71.55 & 84.58 & 84.70 \\
      OFA-L~\cite{wang2022unifying} & RN152 & Embedding layer & 90.05 & \textbf{92.93} & 85.26 & \textbf{85.80} & \textbf{89.87} & \textbf{79.22} & \textbf{85.89} & \textbf{86.55} \\
      \hline
      %PolyFormer-B-1D & Swin-B & BERT-base & 89.53 & 91.92 & 86.52 & 84.26 & 88.11 & 77.71 & 85.01 & 85.60 \\
      %PolyFormer-B-2D & Swin-B & BERT-base & 89.63 & 91.62 & 86.63 & 83.84 & 88.51 & 77.01 & 84.48 & 84.96 \\
      %PolyFormer & Swin-B & BERT-base & 89.27 & 91.89 & 86.52 & 83.57 & 88.00 & 76.74 & 84.46 & 84.61 \\
      PolyFormer-B & Swin-B & BERT-base & 89.73 & 91.73 & 86.03 & 83.73 & 88.60 & 76.38 & 84.46 & 84.96 \\
      %\textbf{PloyFormer} & Swin-L & BERT-base & \textbf{90.35} & 92.81 & \textbf{87.20} & 84.6 & 89.07 & 78.30 & 85.78 & 86.10 \\
      \textbf{PolyFormer-L} & Swin-L & BERT-base & \textbf{90.38} & 92.89 & \textbf{87.16} & 84.98 & 89.77 & 77.97 & 85.83 & 85.91 \\
      %PolyFormer-L-1D & Swin-L & BERT-base & 89.87 & 92.15 & 86.77 & 84.28 & 88.28 & 77.75 & 85.13 & 85.24 \\
      %PolyFormer & Swin-L & BERT-base & 90.35 & 92.81 & 87.20 & 84.6 & 89.07 & 78.30 & 85.78 & 86.10 \\
      \bottomrule[1pt]
   \end{tabular}}}
   \caption{Comparison with the state-of-the-art methods on three referring expression comprehension benchmarks. ENB3 denotes EfficientNet-B3~\cite{tan2019efficientnet}.
%   OFA utilizes
% 19M image-text data for pre-training, while PolyFormer only uses 165K images. 
% \zc{if you want to highlight the best results, all best results should be highlighted if they are not polyformer.} \jl{updated}
}
\vspace{-1.5mm}
   \label{tab:rec}
\end{table*}

==> tables/rec_2.tex <==
\begin{table*}[htbp]
   \centering
    %   \caption{Comparison with state-of-the-art methods in terms of Acc@0.5 on three benchmark datasets for the REC task. Following~\cite{yang2022lavt}, we refer to the language model of each reference method as the main learnable function that transforms word embeddings before multi-modal feature fusion. RN101 and RN152 denotes ResNet-101 and ResNet-152~\cite{he2016deep}, WRN101 refers to Wide ResNet-101~\cite{zagoruyko2016wide}, ENB3 denotes EfficientNetB3~\cite{enb3} and DN53 refers to Darknet-53~\cite{redmon2018yolov3}.}
   \scalebox{0.92}{\setlength{\tabcolsep}{1.5mm}{\begin{tabular}{l|l|l|c|c|c|c|c|c|c|c|c}
      \toprule[1pt]
      \multirow{2}{*}{Method} & Visual &
      Text & \#Pre-train &
      \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
      \cline{5-12}
                                    & Backbone & Encoder & Img-Txt data & val   & test A & test B & val & test A & test B & val & test  \\
      \hline
    %   MAttNet~\cite{yu2018mattnet} & RN101 & Bi-LSTM & 76.65 & 81.14 & 69.99 & 65.33 & 71.62 & 56.02 & 66.58 & 67.27 \\ 
      UNTIER-L~\cite{chen2020uniter} & RN101 & BERT & 4M & 81.41 & 87.04 & 74.17 & 75.90 & 81.45 & 66.70 & 74.86 & 75.77 \\
      VILLA-L~\cite{gan2020large} & RN101 & BERT & 4M & 82.39 & 87.48 & 74.84 & 76.17 & 81.54 & 66.84 & 76.18 & 76.71 \\
      RefTr~\cite{li2021referring} & RN101 & BERT-base & 4.7M & 85.65 & 88.73 & 81.16 & 77.55 & 82.26 & 68.99 & 79.25 & 80.01 \\ 
      UniTAB~\cite{yang2022unitab} & RN101 & RoBERT-base & 1.3M & 86.32 & 88.84 & 80.61 & 78.70 & 83.22 & 69.48 & 79.96 & 79.97 \\
    SeqTR~\cite{zhu2022seqtr} & DN53 & Bi-GRU & 6.1M & 87.00 & 90.15 & 83.59 & 78.69 & 84.51 & 71.87 & 82.69 & 83.37 \\
      MDETR~\cite{kamath2021mdetr} & ENB3 & RoBERTa-base & 4M & 87.51 & 90.40 & 82.67 & 81.13 & 85.52 & 72.96 & 83.35 & 83.31\\
      OFA-B~\cite{wang2022unifying} & RN101 & 
      Embedding layer & 19M & 88.48 & 90.67 & 83.30 & 81.39 & 87.15 & 74.29 & 82.29 & 82.31 \\
      OFA-L~\cite{wang2022unifying} & RN152 & Embedding layer & 19M & 90.05 & \textbf{92.93} & 85.26 & \textbf{85.80} & \textbf{89.87} & \textbf{79.22} & \textbf{85.89} & \textbf{86.55} \\
      \hline
      %PolyFormer-B-1D & Swin-B & BERT-base & 89.53 & 91.92 & 86.52 & 84.26 & 88.11 & 77.71 & 85.01 & 85.60 \\
      %PolyFormer-B-2D & Swin-B & BERT-base & 89.63 & 91.62 & 86.63 & 83.84 & 88.51 & 77.01 & 84.48 & 84.96 \\
      %PolyFormer & Swin-B & BERT-base & 89.27 & 91.89 & 86.52 & 83.57 & 88.00 & 76.74 & 84.46 & 84.61 \\
      PolyFormer & Swin-B & BERT-base & 6M & 89.73 & 91.73 & 86.03 & 83.73 & 88.60 & 76.38 & 84.46 & 84.96 \\
      %\textbf{PloyFormer} & Swin-L & BERT-base & \textbf{90.35} & 92.81 & \textbf{87.20} & 84.6 & 89.07 & 78.30 & 85.78 & 86.10 \\
      \textbf{PolyFormer} & Swin-L & BERT-base & 6M & \textbf{90.38} & 92.89 & \textbf{87.16} & 84.98 & 89.77 & 77.97 & 85.83 & 85.91 \\
      %PolyFormer-L-1D & Swin-L & BERT-base & 89.87 & 92.15 & 86.77 & 84.28 & 88.28 & 77.75 & 85.13 & 85.24 \\
      %PolyFormer & Swin-L & BERT-base & 90.35 & 92.81 & 87.20 & 84.6 & 89.07 & 78.30 & 85.78 & 86.10 \\
      \bottomrule[1pt]
   \end{tabular}}}
   \caption{
   Comparison with the state-of-the-art methods on three referring expression comprehension benchmarks. 
%   OFA utilizes
% 19M image-text data for pre-training, while PolyFormer only uses 165K images. 
% \zc{if you want to highlight the best results, all best results should be highlighted if they are not polyformer.} \jl{updated}
}
   \label{tab:rec}
\end{table*}

==> tables/res.tex <==
\begin{table*}[htbp]
   \centering
    %   \caption{Comparison with state-of-the-art methods in terms of oIoU and mIoU for the RIS task. Following~\cite{yang2022lavt}, we refer to the language model of each reference method as the main learnable function that transforms word embeddings before multi-modal feature fusion. RN101 denotes ResNet-101~\cite{he2016deep}, WRN101 refers to Wide ResNet-101~\cite{zagoruyko2016wide}, and DN53 denotes Darknet-53~\cite{redmon2018yolov3}.}
   \setlength{\tabcolsep}{2.0mm}{\begin{tabular}{ll|l|l|c|c|c|c|c|c|c|c}
      \toprule[1pt]
      & \multirow{2}{*}{Method} & Visual &
      Text & 
      \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
      \cline{5-12}
                                  &  & Backbone & Encoder & val   & test A & test B & val & test A & test B & val & test  \\
      \hline
      %\multicolumn{11}{l}{{oIoU}} \\
      %\hline
      % DMN~\cite{margffoy2018dynamic} & SRU & 49.78 & 54.83 & 45.13 & 38.88 & 44.22 & 32.29 & -     & -      \\
      % RRN~\cite{Li2018rrn}          & LSTM & 55.33 & 57.26 & 53.93 & 39.75 & 42.15 & 36.11 & -     & -      \\
    %   MAttNet~\cite{yu2018mattnet}  & RN101 & Bi-LSTM & 56.51 & 62.37 & 51.70 & 46.67 & 52.39 & 40.08 & 47.64 & 48.61 \\
    %   CMSA~\cite{ye2019cross}       & RN101 & None & 58.32 & 60.61 & 55.09 & 43.76 & 47.60 & 37.89 & -     & -      \\
    %   CAC~\cite{chen2019referring}        & RN101 & Bi-LSTM & 58.90 & 61.77 & 53.81 & -     & -     & -       & 46.37 & 46.95  \\
      & STEP~\cite{chen2019see}       & RN101 & Bi-LSTM & 60.04 & 63.46 & 57.97 & 48.19 & 52.33 & 40.41 & -     & -     \\
      & BRINet~\cite{hu2020bi}    & RN101 & LSTM & 60.98 & 62.99 & 59.21 & 48.17 & 52.32 & 42.11 & -     & -     \\
      & CMPC~\cite{huang2020referring}     & RN101 & LSTM & 61.36 & 64.53 & 59.64 & 49.56 & 53.44 & 43.23 & -     & -      \\
      & LSCM~\cite{hui2020linguistic} & RN101 & LSTM & 61.47 & 64.99 & 59.55 & 49.34 & 53.12 & 43.50 & -     & -      \\
      & CMPC+~\cite{liu2021cross} &  RN101  & LSTM & 62.47 & 65.08 & 60.82 & 50.25 & 54.04 & 43.47 & -     & -     \\
      & MCN~\cite{luo2020multi}       & DN53 & Bi-GRU & 62.44 & 64.20 & 59.71 & 50.62 & 54.99 & 44.69 & 49.22 & 49.40    \\
      & EFN~\cite{EFN}                & WRN101 & Bi-GRU & 62.76 & 65.69 & 59.67 & 51.50 & 55.24 & 43.01 & - & -    \\
      & BUSNet~\cite{yang2021bottom}          & RN101 & Self-Att & 63.27 & 66.41 & 61.39 & 51.76 & 56.87 & 44.13 & - & -  \\
      & CGAN~\cite{luo2020cascade}    & DN53 & Bi-GRU & 64.86 & 68.04 & 62.07 & 51.03 & 55.51 & 44.06 & 51.01 & 51.69 \\
      & LTS~\cite{jing2021locate}   & DN53 & Bi-GRU & 65.43 & 67.76 & 63.08 & 54.21 & 58.32 & 48.02 & 54.40 & 54.25  \\
      % VLT~\cite{Ding_2021_vlt}    &  DN56 & Bi-GRU & 65.65 & 68.29 & 62.73 & 55.50 & 59.20 & 49.36 & 52.99 & 56.65 \\ % mIoU
      & ReSTR~\cite{kim2022restr}  & ViT-B~\cite{dosovitskiy2020image} & Transformer & 67.22 & 69.30 & 64.45 & 55.78 & 60.44 & 48.27 & - & - \\ 
      % LAVT~\cite{yang2022lavt}  & Swin-B & BERT-base & {72.73} & {75.82} & {68.79} & {62.14} & {68.38} & {55.10} & {61.24} & {62.09} \\
      % SeqTR & DN53 & Bi-GRU & 7\\
      \hline
      %PolyFormer  & Swin-B & BERT-base & 74.52 & 76.88 & 71.30 & 68.05 & 72.41 & 60.66 & 67.84 & 69.45 \\
      %PolyFormer & Swin-B & BERT-base & 74.35 & 75.71 & 71.55 & 67.48 & 72.33 & 59.62 & 67.21 & 68.54\\
      %PolyFormer & Swin-B & BERT-base & 74.64 & 77.0 & 71.28 & 67.72 & 72.17 & 60.26 & 67.08 & 68.83\\
      %\textbf{PolyFormer}  & Swin-L & BERT-base & \textbf{76.07} & \textbf{77.84} & \textbf{72.68} & \textbf{69.12} & \textbf{73.88} & \textbf{61.2} & \textbf{68.99} & \textbf{69.96} \\
      & PolyFormer & Swin-B & BERT-base & 74.82 & 76.64 & 71.06 & 67.64 & 72.89 & 59.33 & 67.76 & 69.05\\
      & \textbf{PolyFormer}  & Swin-L & BERT-base & \textbf{75.96} & \textbf{78.29} & \textbf{73.25} & \textbf{69.33} & \textbf{74.56} & \textbf{61.87} & \textbf{69.20} & \textbf{70.19} \\
      % PolyFormer-L-2D (Ours) & Swin-L & BERT-base & 76.07 & 77.84 & 72.68 & 69.12 & 73.88 & 61.2 & 68.99 & 69.96 \\
      
      \hline
      \multicolumn{11}{l}{\textbf{mIoU}} \\
      \hline
      
      & VLT~\cite{ding2021vlt}    &  DN53 & Bi-GRU & 65.65 & 68.29 & 62.73 & 55.50 & 59.20 & 49.36 & 52.99 & 56.65 \\ % mIoU
      & CRIS~\cite{wang2022cris}  & RN101 & GPT-2~\cite{radford2019language} & 70.47 & 73.18 & 66.10 & 62.27 & 68.06 & 53.68 & 59.87 & 60.36 \\ %not sure if it's oIoU or mIoU
      & SeqTR~\cite{zhu2022seqtr} & DN53 & Bi-GRU & 71.70 & 73.31 & 69.82 & 63.04 & 66.73 & 58.97 & 64.69 & 65.74\\
      & RefTr~\cite{li2021referring} & RN101 & BERT-base & 74.34 &76.77 & 70.87 & 66.75 & 70.58 & 59.40 & 66.63 & 67.39 \\
      & LAVT~\cite{yang2022lavt}  & Swin-B & BERT-base & {74.46} & {76.89} & {70.94} & {65.81} & {70.97} & {59.23} & {63.34} & {63.62} \\
    %   RefTr~\cite{li2021referring} & RN101 & BERT-base & 74.34 &76.77 & 70.87 & 66.75 & 70.58 & 59.40 & 66.63 & 67.39 \\
      \hline
      %PolyFormer  & Swin-B & BERT-base & {75.38} &{76.98} & {73.27} & {70.72} & {73.75} & {65.33} & {69.31} & {69.91} \\
      %PolyFormer & Swin-B & BERT-base & 75.10 & 76.51 & 73.21 & 69.95 & 73.72 & 64.81 & 68.55 & 69.17\\
      %PolyFormer-B-1D  & Swin-B & BERT-base & {75.38} &{76.98} & {73.27} & {70.72} & {73.75} & {65.33} & {69.31} & {69.91} \\
      %PolyFormer-B-1D-150 & Swin-B & BERT-base & {75.78} &{77.49} & {73.16} & {71.04} & {74.36} & {65.7} & {68.93} & {69.81} \\
      %PolyFormer-B-2D & Swin-B & BERT-base & 75.10 & 76.51 & 73.21 & 69.95 & 73.72 & 64.81 & 68.55 & 69.17\\
      %PolyFormer & Swin-B & BERT-base & 75.64 & 77.43 & 73.38 & 70.43 & 74.02 & 64.82 & 69.01 & 69.49\\
      %PolyFormer-L-1D & Swin-B & BERT-base & 76.62 & 78.19 & 74.32 & 71.66 & 74.95 & 66.43 & 70.72 & 70.85\\
      & PolyFormer & Swin-B & BERT-base & 75.96 & 77.09 & 73.22 & 70.65 & 74.51 & 64.64 & 69.36 & 69.88\\
      & \textbf{PolyFormer}  & Swin-L & BERT-base  & \textbf{76.94} & \textbf{78.49} & \textbf{74.83} & \textbf{72.15} & \textbf{75.71} & \textbf{66.73} & \textbf{71.15} & \textbf{71.17} \\
      %\textbf{PolyFormer}  & Swin-L & BERT-base  & \textbf{76.98} & \textbf{78.24} & \textbf{74.36} & \textbf{71.96} & \textbf{75.25} & \textbf{66.32} & \textbf{70.76} & \textbf{71.05} \\
      %PolyFormer-L-2D (Ours) & Swin-L & BERT-base & 76.98 & 78.24 & 74.36 & 71.96 & 75.25 & 66.32 & 70.76 & 71.05 \\
      \bottomrule[1pt]
   \end{tabular}}
  \caption{Comparison with the state-of-the-art methods on three referring image segmentation benchmarks. RN101 denotes ResNet-101~\cite{he2016deep}, WRN101 refers to Wide ResNet-101~\cite{zagoruyko2016wide}, and DN53 denotes Darknet-53~\cite{redmon2018yolov3}.}
   \label{tab:res}
%   We report the results of our method with various visual backbones, encoders and decoders. mIoU is utilized as the metric.}
\end{table*}

==> tables/res_v2.tex <==
\begin{table*}[t]
   \centering
    %   \caption{Comparison with state-of-the-art methods in terms of oIoU and mIoU for the RIS task. Following~\cite{yang2022lavt}, we refer to the language model of each reference method as the main learnable function that transforms word embeddings before multi-modal feature fusion. RN101 denotes ResNet-101~\cite{he2016deep}, WRN101 refers to Wide ResNet-101~\cite{zagoruyko2016wide}, and DN53 denotes Darknet-53~\cite{redmon2018yolov3}.}
   \scalebox{0.97}{\setlength{\tabcolsep}{2.0mm}{\begin{tabular}{l|l|l|l|c|c|c|c|c|c|c|c}
      \toprule[1pt]
      %\hline
      \multicolumn{2}{c|}{\multirow{2}{*}{Method}} & Visual &
      Text & 
      \multicolumn{3}{c|}{RefCOCO}  & \multicolumn{3}{c|}{RefCOCO+} & \multicolumn{2}{c}{RefCOCOg} \\
      \cline{5-12}
                                  \multicolumn{2}{c|}{}  & Backbone & Encoder & val   & test A & test B & val & test A & test B & val & test  \\
      \hline
      %\multicolumn{11}{l}{{oIoU}} \\
      %\hline
      % DMN~\cite{margffoy2018dynamic} & SRU & 49.78 & 54.83 & 45.13 & 38.88 & 44.22 & 32.29 & -     & -      \\
      % RRN~\cite{Li2018rrn}          & LSTM & 55.33 & 57.26 & 53.93 & 39.75 & 42.15 & 36.11 & -     & -      \\
    %   MAttNet~\cite{yu2018mattnet}  & RN101 & Bi-LSTM & 56.51 & 62.37 & 51.70 & 46.67 & 52.39 & 40.08 & 47.64 & 48.61 \\
    %   CMSA~\cite{ye2019cross}       & RN101 & None & 58.32 & 60.61 & 55.09 & 43.76 & 47.60 & 37.89 & -     & -      \\
    %   CAC~\cite{chen2019referring}        & RN101 & Bi-LSTM & 58.90 & 61.77 & 53.81 & -     & -     & -       & 46.37 & 46.95  \\
      \multirow{13}{*}{\rotatebox{90}{oIoU}} & STEP~\cite{chen2019see}       & RN101 & Bi-LSTM & 60.04 & 63.46 & 57.97 & 48.19 & 52.33 & 40.41 & -     & -     \\
      & BRINet~\cite{hu2020bi}    & RN101 & LSTM & 60.98 & 62.99 & 59.21 & 48.17 & 52.32 & 42.11 & -     & -     \\
      & CMPC~\cite{huang2020referring}     & RN101 & LSTM & 61.36 & 64.53 & 59.64 & 49.56 & 53.44 & 43.23 & -     & -      \\
      & LSCM~\cite{hui2020linguistic} & RN101 & LSTM & 61.47 & 64.99 & 59.55 & 49.34 & 53.12 & 43.50 & -     & -      \\
      & CMPC+~\cite{liu2021cross} &  RN101  & LSTM & 62.47 & 65.08 & 60.82 & 50.25 & 54.04 & 43.47 & -     & -     \\
      & MCN~\cite{luo2020multi}       & DN53 & Bi-GRU & 62.44 & 64.20 & 59.71 & 50.62 & 54.99 & 44.69 & 49.22 & 49.40    \\
      & EFN~\cite{feng2021encoder}                & WRN101 & Bi-GRU & 62.76 & 65.69 & 59.67 & 51.50 & 55.24 & 43.01 & - & -    \\
      & BUSNet~\cite{yang2021bottom}          & RN101 & Self-Att & 63.27 & 66.41 & 61.39 & 51.76 & 56.87 & 44.13 & - & -  \\
      & CGAN~\cite{luo2020cascade}    & DN53 & Bi-GRU & 64.86 & 68.04 & 62.07 & 51.03 & 55.51 & 44.06 & 51.01 & 51.69 \\
      & LTS~\cite{jing2021locate}   & DN53 & Bi-GRU & 65.43 & 67.76 & 63.08 & 54.21 & 58.32 & 48.02 & 54.40 & 54.25  \\
      % VLT~\cite{Ding_2021_vlt}    &  DN56 & Bi-GRU & 65.65 & 68.29 & 62.73 & 55.50 & 59.20 & 49.36 & 52.99 & 56.65 \\ % mIoU
      & ReSTR~\cite{kim2022restr}  & ViT-B & Transformer & 67.22 & 69.30 & 64.45 & 55.78 & 60.44 & 48.27 & - & - \\ 
      % LAVT~\cite{yang2022lavt}  & Swin-B & BERT-base & {72.73} & {75.82} & {68.79} & {62.14} & {68.38} & {55.10} & {61.24} & {62.09} \\
      % SeqTR & DN53 & Bi-GRU & 7\\
      \cline{2-12}
      %PolyFormer  & Swin-B & BERT-base & 74.52 & 76.88 & 71.30 & 68.05 & 72.41 & 60.66 & 67.84 & 69.45 \\
      %PolyFormer & Swin-B & BERT-base & 74.35 & 75.71 & 71.55 & 67.48 & 72.33 & 59.62 & 67.21 & 68.54\\
      %PolyFormer & Swin-B & BERT-base & 74.64 & 77.0 & 71.28 & 67.72 & 72.17 & 60.26 & 67.08 & 68.83\\
      %\textbf{PolyFormer}  & Swin-L & BERT-base & \textbf{76.07} & \textbf{77.84} & \textbf{72.68} & \textbf{69.12} & \textbf{73.88} & \textbf{61.2} & \textbf{68.99} & \textbf{69.96} \\
      & PolyFormer-B & Swin-B & BERT-base & 74.82 & 76.64 & 71.06 & 67.64 & 72.89 & 59.33 & 67.76 & 69.05\\
      & \textbf{PolyFormer-L}  & Swin-L & BERT-base & \textbf{75.96} & \textbf{78.29} & \textbf{73.25} & \textbf{69.33} & \textbf{74.56} & \textbf{61.87} & \textbf{69.20} & \textbf{70.19} \\
      % PolyFormer-L-2D (Ours) & Swin-L & BERT-base & 76.07 & 77.84 & 72.68 & 69.12 & 73.88 & 61.2 & 68.99 & 69.96 \\
      
      \hline
      %\multicolumn{11}{l}{\textbf{mIoU}} \\
      %\hline
      
      \multirow{7}{*}{\rotatebox{90}{\textbf{mIoU}}} & VLT~\cite{ding2021vlt}    &  DN53 & Bi-GRU & 65.65 & 68.29 & 62.73 & 55.50 & 59.20 & 49.36 & 52.99 & 56.65 \\ % mIoU
      & CRIS~\cite{wang2022cris}  & RN101 & GPT-2 & 70.47 & 73.18 & 66.10 & 62.27 & 68.06 & 53.68 & 59.87 & 60.36 \\ %not sure if it's oIoU or mIoU
      & SeqTR~\cite{zhu2022seqtr} & DN53 & Bi-GRU & 71.70 & 73.31 & 69.82 & 63.04 & 66.73 & 58.97 & 64.69 & 65.74\\
      & RefTr~\cite{li2021referring} & RN101 & BERT-base & 74.34 &76.77 & 70.87 & 66.75 & 70.58 & 59.40 & 66.63 & 67.39 \\
      & LAVT~\cite{yang2022lavt}  & Swin-B & BERT-base & {74.46} & {76.89} & {70.94} & {65.81} & {70.97} & {59.23} & {63.34} & {63.62} \\
    %   RefTr~\cite{li2021referring} & RN101 & BERT-base & 74.34 &76.77 & 70.87 & 66.75 & 70.58 & 59.40 & 66.63 & 67.39 \\
      \cline{2-12}
      %PolyFormer  & Swin-B & BERT-base & {75.38} &{76.98} & {73.27} & {70.72} & {73.75} & {65.33} & {69.31} & {69.91} \\
      %PolyFormer & Swin-B & BERT-base & 75.10 & 76.51 & 73.21 & 69.95 & 73.72 & 64.81 & 68.55 & 69.17\\
      %PolyFormer-B-1D  & Swin-B & BERT-base & {75.38} &{76.98} & {73.27} & {70.72} & {73.75} & {65.33} & {69.31} & {69.91} \\
      %PolyFormer-B-1D-150 & Swin-B & BERT-base & {75.78} &{77.49} & {73.16} & {71.04} & {74.36} & {65.7} & {68.93} & {69.81} \\
      %PolyFormer-B-2D & Swin-B & BERT-base & 75.10 & 76.51 & 73.21 & 69.95 & 73.72 & 64.81 & 68.55 & 69.17\\
      %PolyFormer & Swin-B & BERT-base & 75.64 & 77.43 & 73.38 & 70.43 & 74.02 & 64.82 & 69.01 & 69.49\\
      %PolyFormer-L-1D & Swin-B & BERT-base & 76.62 & 78.19 & 74.32 & 71.66 & 74.95 & 66.43 & 70.72 & 70.85\\
      & PolyFormer-B & Swin-B & BERT-base & 75.96 & 77.09 & 73.22 & 70.65 & 74.51 & 64.64 & 69.36 & 69.88\\
      & \textbf{PolyFormer-L}  & Swin-L & BERT-base  & \textbf{76.94} & \textbf{78.49} & \textbf{74.83} & \textbf{72.15} & \textbf{75.71} & \textbf{66.73} & \textbf{71.15} & \textbf{71.17} \\
      %\textbf{PolyFormer}  & Swin-L & BERT-base  & \textbf{76.98} & \textbf{78.24} & \textbf{74.36} & \textbf{71.96} & \textbf{75.25} & \textbf{66.32} & \textbf{70.76} & \textbf{71.05} \\
      %PolyFormer-L-2D (Ours) & Swin-L & BERT-base & 76.98 & 78.24 & 74.36 & 71.96 & 75.25 & 66.32 & 70.76 & 71.05 \\
      \bottomrule[1pt]
      %\hline
   \end{tabular}}}
  \caption{Comparison with the state-of-the-art methods on three referring image segmentation benchmarks. 
%   \iffalse
  RN101 denotes ResNet-101~\cite{he2016deep}, WRN101 refers to Wide ResNet-101~\cite{zagoruyko2016wide}, and DN53 denotes Darknet-53~\cite{redmon2018yolov3}.
%   \fi
  }
   \label{tab:res}
%   We report the results of our method with various visual backbones, encoders and decoders. mIoU is utilized as the metric.}
\end{table*}
